On the Capacity Region of Bipartite and Tripartite Entanglement Switching

We study a quantum entanglement distribution switch serving a set of users in a star topology with equal-length links. The quantum switch, much like a quantum repeater, can perform entanglement swapping to extend entanglement across longer distances. Additionally, the switch is equipped with entanglement switching logic, enabling it to implement switching policies to better serve the needs of the network. In this work, the function of the switch is to create bipartite or tripartite entangled states among users at the highest possible rates at a fixed ratio. Using Markov chains, we model a set of randomized switching policies. Discovering that some are better than others, we present analytical results for the case where the switch stores one qubit per user, and find that the best policies outperform a time division multiplexing (TDM) policy for sharing the switch between bipartite and tripartite state generation. This performance improvement decreases as the number of users grows. The model is easily augmented to study the capacity region in the presence of quantum state decoherence and associated cut-off times for qubit storage, obtaining similar results. Moreover, decoherence-associated quantum storage cut-off times appear to have little effect on capacity in our identical-link system. We also study a smaller class of policies when the switch stores two qubits per user.

==> C2maxB2ClaimProof.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = bitripartiteToMPECS2020.tex
\begin{proof}
First, we will show that $C_2(r_2,r_3)$ is maximized when $r_2=0$. We prove this by contradiction. When $r_2=0$, $C_2$ is
\begin{align}
C_2(0,r_3)&=
(k-1)\mu\frac{(k-2)(k-1+2r_3)+(k+2r_3)r_3}{(k-2+2r_3)(2k-3+r_3)+(k-1)}.
\label{eq:C2r20r3}
\end{align}
Suppose that there exists some value of $r_2\neq 0$ that yields a larger value of $C_2$, \ie, for some $r_2\in (0,1]$,
\begin{align*}
&(k-1)\mu\frac{(k-2)\bar{r}_2[k(3k-2)(k-1+2r_3)+(k-2)r_2((k-1)((k+1)(k-2)+2kr_3)+3k-2)]}{D_2}\\
&\quad+(k-1)\mu\frac{(3k-2)k(k+2r_3)r_3}{D_2}
> (k-1)\mu\frac{(k-2)(k-1+2r_3)+(k+2r_3)r_3}{(k-2+2r_3)(2k-3+r_3)+(k-1)},
\end{align*}
or, after dividing by $(k-1)\mu$ and simplifying the left-hand side,
\begin{align}
&\frac{(k-2)k\bar{r}_2[(3k-2)(k-1+2r_3)+(k-2)r_2(k^2-2(k-1)(1-r_3))]}{D_2}\nonumber\\
&\quad+\frac{(3k-2)k(k+2r_3)r_3}{D_2}
> \frac{(k-2)(k-1+2r_3)+(k+2r_3)r_3}{(k-2+2r_3)(2k-3+r_3)+(k-1)}.
\end{align}
By Lemmas \ref{lemma:C2proofpart1} and \ref{lemma:C2proofpart2}, this is a contradiction. Thus, $r_2=0$ yields the maximum value of $C_2$. 

Next, we use a similar argument to prove that $r_3=1$ maximizes (\ref{eq:C2r20r3}). We have
\begin{align*}
C_2(0,1) &= \frac{k^2\mu}{2k+1}.
\end{align*}
Suppose that there exists some value of $r_3\neq 1$ that achieves a higher value of $C_2$. In other words, there exists some $r_3\in[0,1)$ such that
\begin{align*}
(k-1)\mu\frac{(k-2)(k-1+2r_3)+(k+2r_3)r_3}{(k-2+2r_3)(2k-3+r_3)+(k-1)} &> \frac{k^2\mu}{2k+1},
\end{align*}
or, after expanding, simplifying, and collecting terms by $k$,
\begin{align*}
-(1-r_3)k^3 + (2r_3^2 - 3r_3 + 1)k^2 + (- 2r_3^2 + r_3 + 1)k - 2r_3^2 + 4r_3 - 2 &>0.
\end{align*}
We have a contradiction by Lemma \ref{lemma:C2proofpart3}, completing the proof that $(r_2,r_3)=(0,1)$ maximizes $C_2$.
\end{proof}

\begin{lemma}
\label{lemma:C2proofpart1}
For $k\geq 2$, $r_2\in(0,1]$, and $r_3\in[0,1]$,
\begin{align}
\frac{(3k-2)k(k+2r_3)r_3}{D_2} \leq \frac{(k+2r_3)r_3}{(k-2+2r_3)(2k-3+r_3)+(k-1)}.
\label{eq:lemmaC2proofpart1}
\end{align}
\end{lemma}
\begin{proof}
Clearly, (\ref{eq:lemmaC2proofpart1}) holds when $r_3=0$. When $r_3\in(0,1]$, (\ref{eq:lemmaC2proofpart1}) is equivalent to
\begin{align}
&\frac{(3k-2)k}{D_2} \leq \frac{1}{(k-2+2r_3)(2k-3+r_3)+(k-1)}.
\label{eq:lemmaC2proofpart1_2}
\end{align}
Note that for $r_2\in (0,1]$, we can see from Remark \ref{remark:D2} (see below) that
\begin{align*}
D_2 %&= (k-1)(k-2)[k(2kr_3+(k+1)(k-2))-(k-2+2r_3)(3k-2)]r_2^2\\
%&\quad+k[(2kr_3+(k+1)(k-2))(2(k-1)^2+k-2)-(2k-3)(k-2+2r_3)(3k-2)]r_2\\
%&\quad+(k-2+2r_3)(3k-2)(k(2k-3)+kr_3)+k(k-1)(3k-2)\\
&> (k-2+2r_3)(3k-2)(k(2k-3)+kr_3)+k(k-1)(3k-2).
\end{align*}
Thus, to show that (\ref{eq:lemmaC2proofpart1_2}) holds, it would suffice to show that
\begin{align*}
(3k-2)k[(k-2+2r_3)(2k-3+r_3)+&(k-1)]\\
&\leq (k-2+2r_3)(3k-2)(k(2k-3)+kr_3)+k(k-1)(3k-2),\\
(k-2+2r_3)(2k-3+r_3)+(k-1)&\leq (k-2+2r_3)(2k-3+r_3)+(k-1),
\end{align*}
which is clearly true.
\end{proof}
\begin{lemma}
\label{lemma:C2proofpart2}
For $k\geq 2$, $r_2\in(0,1]$, and $r_3\in[0,1]$,
\begin{align}
&\frac{k\bar{r}_2[(3k-2)(k-1+2r_3)+(k-2)r_2(k^2-2(k-1)(1-r_3))]}{D_2}
< \frac{(k-1+2r_3)}{(k-2+2r_3)(2k-3+r_3)+(k-1)}.
\label{eq:C2proofpart2}
\end{align}
\end{lemma}
\begin{proof}
To prove (\ref{eq:C2proofpart2}), we first simplify the problem by removing the negative term from the numerator of the left-hand side. In other words, to show that (\ref{eq:C2proofpart2}) holds, it suffices to prove that the following holds:
\begin{align*}
&\frac{\bar{r}_2[(3k-2)k(k-1+2r_3)+(k-2)k^3r_2]}{D_2}< \frac{(k-1+2r_3)}{(k-2+2r_3)(2k-3+r_3)+(k-1)}.
\end{align*}
Expanding the left-hand side numerator of the inequality above yields
\begin{align*}
&\frac{(3k-2)k(k-1+2r_3)+k[(k-2)k^2-(3k-2)(k-1+2r_3)]r_2-(k-2)k^3r_2^2}{D_2}\\
&\qquad< \frac{(k-1+2r_3)}{(k-2+2r_3)(2k-3+r_3)+(k-1)},
\end{align*}
or
\begin{align}
&\left((3k-2)k(k-1+2r_3)+k[(k-2)k^2-(3k-2)(k-1+2r_3)]r_2-(k-2)k^3r_2^2\right)D_2\lvert_{r_2=0}\nonumber\\
&\qquad\qquad< (k-1+2r_3)D_2,
\label{eq:C2proofpart2_1}
\end{align}
where $D_2\lvert_{r_2=0} \coloneqq (k-2+2r_3)(2k-3+r_3)+(k-1)$. Note from Remark \ref{remark:D2} that the right-hand side of (\ref{eq:C2proofpart2_1}) has the term 
\begin{align}
(k-1+2r_3)[(k-2+2r_3)(3k-2)(k(2k-3)+kr_3)+k(k-1)(3k-2)],
\label{eq:C2proofpart2_2}
\end{align}
equal to the term $(3k-2)k(k-1+2r_3)D_2\lvert_{r_2=0}$ on the left-hand side of (\ref{eq:C2proofpart2_1}). To see this, first divide both of these terms by $(3k-2)k(k-1+2r_3)$, which for (\ref{eq:C2proofpart2_2}) yields
\begin{align*}
(k-2+2r_3)(2k-3+kr_3)+(k-1),
\end{align*}
which equals $D_2\lvert_{r_2=0}$. Thus, proving (\ref{eq:C2proofpart2_1}) amounts to proving that
\begin{align}
&\left(k[(k-2)k^2-(3k-2)(k-1+2r_3)]r_2-(k-2)k^3r_2^2\right)D_2\lvert_{r_2=0}< (k-1+2r_3)R,
\label{eq:C2proofpart2_3}
\end{align}
where $R\coloneqq D_2 - (3k-2)k(k-1+2r_3)D_2\lvert_{r_2=0}$. We can simplify the task even further by removing the negative term with the $r_2^2$ coefficient from the left side of the inequality, and then arguing that the terms with $r_2$ on the left-hand side are smaller than those with $r_2$ on the right side. Note that there is still a term with $r_2^2$ on the right side of (\ref{eq:C2proofpart2_3}), but it is positive (see Remark \ref{remark:D2}). Thus, we must show that
\begin{align*}
&k[(k-2)k^2-(3k-2)(k-1+2r_3)][(k-2+2r_3)(2k-3+r_3)+(k-1)]r_2 \\
&\quad<(k-1+2r_3)k[(2kr_3+(k+1)(k-2))(2(k-1)^2+k-2)-(2k-3)(k-2+2r_3)(3k-2)]r_2,
\end{align*}
or, by dividing by $kr_2$ (allowed since $r_2\neq 0$),
\begin{align*}
&[(k-2)k^2-(3k-2)(k-1+2r_3)][(k-2+2r_3)(2k-3+r_3)+(k-1)] \\
&\quad<(k-1+2r_3)[(2kr_3+(k+1)(k-2))(2(k-1)^2+k-2)-(2k-3)(k-2+2r_3)(3k-2)].
%&[5k + 4r_3 - 6kr_3 - 5k^2 + k^3 - 2][(k-2+2r_3)(2k-3+r_3)+(k-1)] \\
%&\quad<(k-1+2r_3)[(2kr_3+(k+1)(k-2))k-(k-2+2r_3)(3k-2)](2k-3),\\
\end{align*}
Expanding and simplifying yields
\begin{align*}
- 3(r_3 +1)k^4 + (- 6r_3^2 - r_3 + 10)k^3 + (- 4r_3^2 + 17r_3 - 9)k^2 + (- 12r_3^3 + 26r_3^2 - 14r_3 - 1)k& + 8r_3^3 - 12r_3^2 + 2,
\end{align*}
which should be negative.

Let us examine the term $f(r_3) \coloneqq - 12r_3^3 + 26r_3^2 - 14r_3$ and see if it is negative for $r_3\in[0,1]$:
\begin{align*}
f(r_3)= 2(- 6r_3^2 + 13r_3 - 7) = 2(1-r_3)(6r_3-7).
\end{align*}
Clearly, this quantity is always negative for the given interval of $r_3$, so to simplify our task, we can simply remove it from the inequality. Similarly, the term $8r_3^3 - 12r_3^2 = 4r_3^2(2r_3-3)$ is also negative for $r_3\in[0,1]$ and can also be removed.
It then suffices to prove that
\begin{align*}
- 3(r_3 +1)k^4 + (- 6r_3^2 - r_3 + 10)k^3 + (- 4r_3^2 + 17r_3 - 9)k^2 -k  + 2 &<0.
\end{align*}
The term $-k+2$ is negative for $k\geq 2$ and thus may also be removed, so that it suffices to prove
\begin{align}
- 3(r_3 +1)k^2 + (- 6r_3^2 - r_3 + 10)k + (- 4r_3^2 + 17r_3 - 9) &<0.
\label{eq:C2proofpart2_4}
\end{align}
Differentiating the left-hand side of (\ref{eq:C2proofpart2_4}) with respect to $k$ yields 
%$- 6(r_3 +1)k + (- 6r_3^2 - r_3 + 10)$ and a critical point at
%\begin{align}
%k =\frac{ 10-6r_3^2 - r_3}{6(r_3 +1)},
%\label{eq:C2proofpart2_5}
%\end{align}
%which is a global maximum (by the second derivative test). However, the maximum value of (\ref{eq:C2proofpart2_5}) is achieved when $r_3=0$, yielding $k=10/6$, which is outside the acceptable interval for $k$ as it is less than two. On the other hand, 
\begin{align*}
- 6(r_3 +1)k + (- 6r_3^2 - r_3 + 10) = - 6r_3k  - 6r_3^2 - r_3 + 10 - 6k,
\end{align*}
which is negative for $k\geq 2$, indicating that the function is decreasing in $k$. Thus, if the left-hand side of (\ref{eq:C2proofpart2_4}) is negative for $k=2$, then it would follow that it is also negative for $k>2$. When $k=2$, the left side of (\ref{eq:C2proofpart2_4}) is
\begin{align*}
- 16r_3^2 + 3r_3 - 1,
\end{align*}
whose derivative with respect to $r_3$ is $-32r_3+3$, yielding a global maximum at $3/32$, at which point the function evaluates to $-55/64$.
\end{proof}

\begin{remark}
\label{remark:D2}
Following are some useful properties of $D_2$, the denominator of $C_2$ and $C_3$ for buffer size-two systems.
\end{remark}
Let us group the terms of the denominator of $C_2$ and $C_3$ by $r_2$, so that it becomes
\begin{align}
D_2 &= (k-1)(k-2)[k(2kr_3+(k+1)(k-2))-(k-2+2r_3)(3k-2)]r_2^2\nonumber\\
&\quad+k[(2kr_3+(k+1)(k-2))(2(k-1)^2+k-2)-(2k-3)(k-2+2r_3)(3k-2)]r_2\nonumber\\
&\quad+(k-2+2r_3)(3k-2)(k(2k-3)+kr_3)+k(k-1)(3k-2).
\label{eq:D2r2}
\end{align}
It is easy to see that the terms above that do not depend on $r_2$ are positive (recall that $k\geq 2$ and $r_3\in[0,1]$).
To show that the term with the $r_2^2$ coefficient is also positive, it suffices to show that
\begin{align*}
k(2kr_3+(k+1)(k-2))&>(k-2+2r_3)(3k-2),~\quad\text{or equivalently, that}\\
2k^2r_3+k^3-k^2-2k&>3k^2-8k+4+6kr_3-4r_3,\\
%2(k-2)(k-1)r_3+k^3-4k^2+6k-4&>0,\\
2(k-2)(k-1)r_3+(k-2)(k^2-2k+2)&>0,\\
2(k-1)r_3+k^2-2k+2&>0,
\end{align*}
which is clearly satisfied for $k\geq 2$. Finally, for the coefficient of $r_2$ to be positive, we require that
\begin{align*}
(2kr_3+(k+1)(k-2))(2(k-1)^2+k-2)-(2k-3)(k-2+2r_3)(3k-2) &>0,\\
(2kr_3+(k+1)(k-2))(2k-3)k-(2k-3)(k-2+2r_3)(3k-2) &>0,\\
%2k^2r_3+k^3-k^2-2k-6kr_3 + 4r_3 + 8k - 3k^2 - 4 &>0,\\
2r_3(k^2-3k + 2)+k^3 - 4k^2 + 6k  - 4 &>0,\\
2r_3(k-2)(k-1)+(k-2)(k^2-2k+2) &>0,\\
2r_3(k-1)+k^2-2k+2 &>0
\end{align*}
The left-hand side of this inequality is positive; thus, the coefficient of $r_2$ is also positive.

\begin{lemma}
For $k\geq 2$ and $r_3\in[0,1)$,
\begin{align}
-(1-r_3)k^3 + (2r_3^2 - 3r_3 + 1)k^2 + (- 2r_3^2 + r_3 + 1)k - 2r_3^2 + 4r_3 - 2 &<0.
\label{eq:C2proofpart3_1}
\end{align}
\label{lemma:C2proofpart3}
\end{lemma}
\begin{proof}
First, consider the term in (\ref{eq:C2proofpart3_1}) that does not depend on $k$:
\begin{align*}
- 2r_3^2 + 4r_3 - 2 = - 2(r_3^2 - 2r_3 + 1)=-2(r_3-1)^2
\end{align*}
and note that it is always negative. Thus, to prove (\ref{eq:C2proofpart3_1}) it would suffice to prove that
\begin{align}
-(1-r_3)k^3 + (2r_3^2 - 3r_3 + 1)k^2 + (- 2r_3^2 + r_3 + 1)k &<0,\nonumber\\
-(1-r_3)k^2 + (2r_3^2 - 3r_3 + 1)k - 2r_3^2 + r_3 + 1 &<0.
\label{eq:C2proofpart3_2}
\end{align}
Differentiating the left-hand side with respect to $k$ yields
\begin{align}
-2(1-r_3)k + 2r_3^2 - 3r_3 + 1 = 2r_3^2+(2k-3)r_3 + 1-2k.
\label{eq:C2proofpart3_3}
\end{align}
Since $2k-3$ is positive for $k\geq 2$, (\ref{eq:C2proofpart3_3}) is increasing in $r_3$, so $r_3=1$ maximizes it at a value of $0$. Thus, for $r_3\in[0,1)$, (\ref{eq:C2proofpart3_3}) is negative, implying that (\ref{eq:C2proofpart3_2}) is decreasing in $k$. For $k=2$, (\ref{eq:C2proofpart3_3}) is
\begin{align*}
-4+4r_3 + 4r_3^2 - 6r_3 + 2 - 2r_3^2 + r_3 + 1=2r_3^2 - r_3-1,
\end{align*}
which is negative between $r_3=-1/2$ and $r_3=1$.
\end{proof}


==> C3FarthestPoint.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = bitripartiteToMPECS2020.tex
\begin{proof}
The proof is similar to that of the $B=1$ case (see Section \ref{sec:B1analysis}): it is sufficient to find the point $(C_3,C_2)$ that maximizes the quantity $\lvert C_2-C_2^*(1-C_3/C_3^*)\rvert$
\end{proof}

==> C3maxB2ClaimProof.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = bitripartiteToMPECS2020.tex
\begin{proof}
First, we show that $C_3(r_2,r_3)$  is maximized when $r_2=1$. To see this, first note that $C_3(0,r_3)=0$. Then, defining
\begin{align*}
A&\coloneqq k(3k-2)(k-1+2r_3),\\
B&\coloneqq (k-2)[(k-1)((k+1)(k-2)+2kr_3)+3k-2],
\end{align*}
and differentiating $C_3$ with respect to $r_2$ yield
\begin{align}
\frac{\partial C_3}{\partial r_2} = (k-1)(k-2)\mu \frac{(A+2Br_2)D_2-r_2(A+Br_2)\frac{\partial D_2}{\partial r_2}}{D_2^2}.
\label{eq:C3proof1}
\end{align}
Let
\begin{align*}
D_2 &= Er_2^2+Fr_2+G,
\end{align*}
where $E$, $F$, and $G$ are given by (\ref{eq:D2r2}) and are positive. Note that $A$ and $B$ are also positive. Then (\ref{eq:C3proof1}) can be rewritten as
\begin{align*}
\frac{\partial C_3}{\partial r_2} &= (k-1)(k-2)\mu \frac{(A+2Br_2)(Er_2^2+Fr_2+G)-(A+Br_2)(2Er_2^2+Fr_2)}{D_2^2}\\
&= (k-1)(k-2)\mu \frac{-AEr_2^2+BFr_2^2+(A+2Br_2)G}{D_2^2},
\end{align*}
and our goal is to show that this quantity is positive (since this would imply that $C_3$ is increasing with $r_2$, and thus is maximized at $r_2=1$). To prove this, it suffices to show that $BF-AE\geq 0$ when $k\geq 2$. Let $H\coloneqq2kr_3+(k+1)(k-2)$, $I\coloneqq(k-2+2r_3)(3k-2)$, and note that $kH-I = (k - 2)(2r_3(k - 1)  + k^2- 2k + 2)$ is positive for $k\geq 2$. 
It can be shown that
\begin{align*}
BF-AE&=k(k-2)(2k-3)[(k-1)H+3k-2][kH-I]\\
&\quad-k(3k-2)(k-1+2r_3)(k-1)(k-2)[kH-I]\\
&=k(kH-I)(k-2)[(2k-3)\left((k-1)H+3k-2\right)-(3k-2)(k-1+2r_3)(k-1)]\\
&=k(kH-I)(k-2)(2k^4 + (4r_3 - 10)k^3 + (18 - 16r_3)k^2 + (16r_3 - 13)k - 4r_3 + 2).
\end{align*}
When $k=2$, it is easy to see that $BF-AE=0$. For $k\geq 3$, we need only to focus on the third expression in the parentheses above, since $k(kH-I)(k-2)>0$. Let 
\begin{align*}
f(k)=2k^4 + (4r_3 - 10)k^3 + (18 - 16r_3)k^2 + (16r_3 - 13)k - 4r_3 + 2.
\end{align*}
Next, we have $f(r_3)=17+8r_3$ and 
\begin{align*}
f^{\prime}(k)&=8k^3 + 3(4r_3 - 10)k^2 + 2(18 - 16r_3)k + (16r_3 - 13)\\
&=(12k^2 - 32k + 16)r_3 + 8k^3 - 30k^2 + 36k - 13\\
&=4(3k-2)(k-2)r_3 + 8(k-1)^3-6(k-1)^2+1,
\end{align*}
which is easily seen to be positive for $k\geq 3$, implying that $f(k)$ is increasing when $k\geq 3$. This completes the proof that $C_3$ is maximized when $r_2=1$. Next, we prove that $C_3(1,r_3)$ is maximized at $r_3=0$.
\begin{align*}
C_3(1,0) &=  \frac{k(k-1)(k-2)\mu\left((3k-2)(k-1)+(k-2)(k^2-2k+2)\right)}{k(k+1)(k-2)(3k(k-2)+2)-(k-2)^2(3k-2)(k-1)+k(k-1)(3k-2)}.
\end{align*}
Suppose for a contradiction that there exists some $r_3\in (0,1]$ that yields a larger value for $C_3$ than $C_3(1,0)$. In other words, $C_3(1,0)<C_3(1,r_3)$ for an $r_3\in (0,1]$, or
\begin{align*}
&\frac{k(3k-2)(k-1)+k(k-2)(k^2-2k+2)}{k(k+1)(k-2)(3k(k-2)+2)-(k-2)^2(3k-2)(k-1)+k(k-1)(3k-2)}\\
&<\frac{k(3k-2)(k-1+2r_3)+(k-2)[(k-1)((k+1)(k-2)+2kr_3)+3k-2]}{D_2(r_2=1,r_3)}.
\end{align*}
By Lemmas \ref{lemma:C3lemma4} and \ref{lemma:C3lemma5}, this is a contradiction.
\end{proof}
\begin{lemma}\label{lemma:C3lemma4}
For $k\geq 2$ and $r_3\in(0,1]$,
\begin{align}
\frac{(k-1)}{k(k+1)(k-2)(3k(k-2)+2)-(k-2)^2(3k-2)(k-1)+k(k-1)(3k-2)}>\frac{(k-1+2r_3)}{D_2(r_2=1,r_3)}.
\label{eq:lemma4statement}
\end{align}
\end{lemma}
\begin{proof}
Note that the denominator of the left-hand side of (\ref{eq:lemma4statement}) is $D_2(r_2=1,r_3=0)$ (which, of course, is positive for $k\geq 2$), so
to prove (\ref{eq:lemma4statement}), we must show that
\begin{align*}
(k-1)D_2(r_2=1,r_3)>(k-1+2r_3)D_2(r_2=1,r_3=0),
\end{align*}
which simplifies to
\begin{align}
r_3(4kr_3 - 24k - 10k^2r_3 + 6k^3r_3 + 20k^2 - 11k^3 + 3k^4 + 8) > 0.
\label{eq:lemma4_2}
\end{align}
Using the assumption that $r_3\in (0,1]$, we can divide (\ref{eq:lemma4_2}) by $r_3$ and rewrite it as
\begin{align}
2k(3k-2)(k-1)r_3 + (k - 2) (3 k^3 - 5 k^2 + 10 k - 4) >0.
\label{eq:lemma4_3}
\end{align}
Again using the assumption that $r_3\in (0,1]$, it is easy to see that $2k(3k-2)(k-1)r_3$ is strictly positive for $k\geq 2$. Meanwhile, the remaining portion of (\ref{eq:lemma4_3}) is either 0 (when $k=2$) or positive (for $k\geq 3$). To see the latter, note that
\begin{align*}
3 k^3 - 5 k^2 + 10 k - 4 = k^2(3k-5)+2(5k-2)
\end{align*}
is positive for $k=3$ and increasing with $k$ in the interval $k\geq 3$.
\end{proof}
\begin{lemma}\label{lemma:C3lemma5}
For $k\geq 2$ and $r_3\in(0,1]$,
\begin{align}
\frac{k(k^2-2k+2)}{D_2(r_2=1,r_3=0)}>\frac{(k-1)((k+1)(k-2)+2kr_3)+3k-2}{D_2(r_2=1,r_3)},
\label{eq:lemma5statement}
\end{align}
where $D_2(r_2=1,r_3=0)=k(k+1)(k-2)(3k(k-2)+2)-(k-2)^2(3k-2)(k-1)+k(k-1)(3k-2)$.
\end{lemma}
\begin{proof}
Simplifying (\ref{eq:lemma5statement}) yields
\begin{align*}
k^2r_3(3k - 2)(4k + 4r_3 - 4kr_3 + 2k^2r_3 - 2k^2 + k^3 - 6) >0,
\end{align*}
or, after diving by $r_3$ (since $r_3\in(0,1]$) and grouping terms by $r_3$,
\begin{align*}
(2k(k-2)+4)r_3 + k ((k - 2) k + 4) - 6 >0.
\end{align*}
It is easy to see that the left-hand side is positive for $k=2$ and increasing for $k\geq 2$.
\end{proof}
